Measurement of the ratio of branching fractions $\mathcal{B}(B_c^+\,\to\,J/\psi\tau^+\nu_\tau)$/$\mathcal{B}(B_c^+\,\to\,J/\psi\mu^+\nu_\mu)$

A measurement is reported of the ratio of branching fractions $\mathcal{R}(J/\psi)=\mathcal{B}(B_c^+\,\to\,J/\psi\tau^+\nu_\tau)/\mathcal{B}(B_c^+\,\to\,J/\psi \mu^+\nu_\mu)$, where the $\tau^+$ lepton is identified in the decay mode $\tau^+\,\to\,\mu^+\nu_\mu\overline{\nu}_\tau$. This analysis uses a sample of proton-proton collision data corresponding to 3.0$\mathrm{\,fb}^{-1}$ of integrated luminosity recorded with the LHCb experiment at center-of-mass energies $7\,\mathrm{TeV}$ and $8\,\mathrm{TeV}$. A signal is found for the decay $B_c^+\,\to\,J/\psi \tau^+\nu_\tau$ at a significance of 3 standard deviations, corrected for systematic uncertainty, and the ratio of the branching fractions is measured to be $\mathcal{R}(J/\psi) = 0.71 \pm 0.17 \mathrm{\,(stat)} \pm 0.18\mathrm{\,(syst)}$. This result lies within 2 standard deviations above the range of existing predictions in the Standard Model.

==> LHCb_authorlist.tex <==
% $Id: LHCb_authorlist.tex 78711 2015-08-06 07:54:32Z apuignav $
% ===============================================================================
% Purpose: example of authorlist for LHCb template
% Author:
% Created on: 2009-09-24
% ===============================================================================

%\documentclass[a4paper]{article}
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm}
%\setlength{\textwidth}{16.5cm}
%\setlength{\parindent}{0cm}
%\begin{document}
\centerline{\large\normalfont\bfseries LHCb collaboration}
\begin{flushleft}
\small
%-- LHCb Authorlist, Example typesetting
%-- 
A.~N.~Other$^{1}$.\bigskip\newline{\it
\footnotesize
$ ^{1}$University of nowhere\\
}
%-- 
%-- 
\end{flushleft}
%\end{document}

